ML-Bench: Evaluating Large Language Models and Agents for Machine Learning Tasks on Repository-Level Code

Despite Large Language Models (LLMs) like GPT-4 achieving impressive results in function-level code generation, they struggle with repository-scale code understanding (e.g., coming up with the right arguments for calling routines), requiring a deeper comprehension of complex file interactions. Also, recently, people have developed LLM agents that attempt to interact with repository code (e.g., compiling and evaluating its execution), prompting the need to evaluate their performance. These gaps have motivated our development of ML-Bench, a benchmark rooted in real-world programming applications that leverage existing code repositories to perform tasks. Addressing the need for LLMs to interpret long code contexts and translate instructions into precise, executable scripts, ML-Bench encompasses annotated 9,641 examples across 18 GitHub repositories, challenging LLMs to accommodate user-specified arguments and documentation intricacies effectively. To evaluate both LLMs and AI agents, two setups are employed: ML-LLM-Bench for assessing LLMs' text-to-code conversion within a predefined deployment environment, and ML-Agent-Bench for testing autonomous agents in an end-to-end task execution within a Linux sandbox environment. Our findings indicate that while GPT-4o leads with a Pass@5 rate surpassing 50%, there remains significant scope for improvement, highlighted by issues such as hallucinated outputs and difficulties with bash script generation. Notably, in the more demanding ML-Agent-Bench, GPT-4o achieves a 76.47% success rate, reflecting the efficacy of iterative action and feedback in complex task resolution. Our code, dataset, and models are available at https://github.com/gersteinlab/ML-bench.

==> files/11-datasheet.tex <==
\thispagestyle{plain}
\newcommand{\edit}[1]{#1}

\clearpage
\section{Data Sheet}

\subsection{Motivation}

The questions in this section are primarily intended to encourage
dataset creators to clearly articulate their reasons for creating the
dataset and to promote transparency about funding interests.
The latter may be particularly relevant for datasets created for
research purposes.\\

% 

\paragraph{For what purpose was the dataset created?}
Was there a specific task in mind? Was there a specific gap that needed to be filled? Please provide a description.

Despite LLMs like GPT-4 achieving impressive results in function-level code generation, they struggle with repository-scale code understanding (e.g., coming up with the right arguments for calling routines), requiring a deeper comprehension of complex file interactions.
So a gap exists between the function-level code generation and repository-scale code understanding tasks, which needs filling.
Also, recently, people have developed LLM agents that attempt to interact with repository code (e.g., compiling and evaluating its execution), prompting the need to evaluate their performance.  
These gaps have motivated our development of \textsc{ML-Bench}, a benchmark rooted in real-world programming applications that leverage existing code repositories to perform tasks. 

\paragraph{Who created the dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organization)?}

Yale University, Zhejiang University, and Peking University created the dataset on behalf of Yale University, Zhejiang University, and Peking University.

\paragraph{ \textbf{}Who funded the creation of the dataset?}

If there is an associated grant, please provide the name of the grantor and the grant name and number.

Xiangru Tang, Yanjun Shao and Mark Gerstein are supported by Schmidt Futures.

\paragraph{Any other comments?}

No.

% 

\subsection{Composition}

Dataset creators should read through \edit{these questions} prior to
any data collection and then provide answers once \edit{data} collection is
complete. Most of the questions \edit{in this section} are intended to
provide dataset consumers with the information they need to make
informed decisions about using the dataset for their chosen
tasks. Some of the questions are \edit{designed to elicit} information
about compliance with the EU's General Data Protection Regulation
(GDPR) or comparable regulations in other jurisdictions.

\edit{Questions that apply only to datasets that relate to people are
grouped together at the end of the section. We recommend broadening the
interpretation of whether a dataset relates to people. For
example, any dataset containing text that was written by people
relates to people.}\\

% 

\paragraph{What do the instances that comprise the dataset
    represent (e.g., documents, photos, people, countries)?} Are there
  multiple types of instances (e.g., movies, users, and ratings;
  people and interactions between them; nodes and edges)? Please
  provide a description.

The instance in this dataset is a specific task about how to use a repository with its corresponding code.

\paragraph{How many instances are there in total (of each type, if appropriate)?}

\textsc{ML-Bench} encompasses annotated \textbf{9,641} examples across \textbf{18} GitHub repositories

\paragraph{Does the dataset contain all possible instances, or is it
    a sample (not necessarily random) of instances from a larger set?}
  If the dataset is a sample, then what is the larger set? Is the
  sample representative of the larger set (e.g., geographic coverage)?
  If so, please describe how this representativeness was
  validated/verified. If it is not representative of the larger set,
  please describe why not (e.g., to cover a more diverse range of
  instances, because instances were withheld or unavailable).

The dataset contains all possible instances.

\paragraph{What data does each instance consist of?} ``Raw'' data
  (e.g., unprocessed text or images) or features? In either case,
  please provide a description.

  Each instance consist of a repository, the instruction about a task that can be finished using this repository, and the ground truth code to finish the task.

\paragraph{Is there a label or target associated with each
    instance?} If so, please provide a description.

Yes, the label associated with each instance is a code snippet that can fulfill the instruction.

\paragraph{Is any information missing from individual instances?}
  If so, please provide a description explaining why this information
  is missing (e.g., because it was unavailable). This does not include
  intentionally removed information but might include, e.g., redacted
  text.

  No.

\paragraph{Are relationships between individual instances made
    explicit (e.g., users' movie ratings, social network links)?} If
  so, please describe how these relationships are made explicit.

There are no relationships between individual instances.

\paragraph{Are there recommended data splits (e.g., training,
    development/validation, testing)?} If so, please provide a
  description of these splits, explaining the rationale behind them.

Yes, there are recommended data splits.
We construct ML-Bench from 18 diverse repositories, each reflecting varying complexity and tasks, while filtering out substandard samples. Regarding the code language, our annotated output includes both \textbf{bash scripts}, which invoke Python files with specific arguments, and \textbf{Python code}, which calls functions directly from the repository. Bash scripts significantly outnumbered Python code snippets.

On average, each repository contributed approximately 480 examples, summing up to 9,641 examples.
For our experiments involving the fine-tuning of open-source LLMs, we split the dataset based on code origin: The \textbf{In-Distribution (ID)} approach utilizes data from the same repository both for training and testing, allowing repository-specific code to be exposed to models during fine-tuning. In contrast, the \textbf{Out-Of-Distribution (OOD)} method employs disjoint sets for training and testing, encompassing eight repositories—half for model training and the remaining for evaluation.



\paragraph{Are there any errors, sources of noise, or redundancies
    in the dataset?} If so, please provide a description.

No.

\paragraph{Is the dataset self-contained, or does it link to or
    otherwise rely on external resources (e.g., websites, tweets,
    other datasets)?} If it links to or relies on external resources,
    a) are there guarantees that they will exist and remain constant,
    over time; b) are there official archival versions of the complete
    dataset (i.e., including the external resources as they existed at
    the time the dataset was created); c) are there any restrictions
    (e.g., licenses, fees) associated with any of the external
    resources that might apply to a \edit{dataset consumer}? Please provide
    descriptions of all external resources and any restrictions
    associated with them, as well as links or other access points, as
    appropriate.

    Each sample in the dataset is linked to a GitHub repository. We provide all linked GitHub repository in our open-source codebase. The official archival versions of the complete dataset is provided in our open-source openbase.The restriction associated with any of the external resources is provided at Appendix B.

\paragraph{Does the dataset contain data that might be considered
    confidential (e.g., data that is protected by legal privilege or
    by doctor\edit{--}patient confidentiality, data that includes the content
    of individuals' non-public communications)?} If so, please provide
    a description.

No.

\paragraph{Does the dataset contain data that, if viewed directly,
    might be offensive, insulting, threatening, or might otherwise
    cause anxiety?} If so, please describe why.

No.

\edit{If the dataset does not }relate to people, you may skip the remaining questions in this section.

The dataset does not relate to people, so we skip the remaining questions.

\paragraph{Does the dataset identify any subpopulations (e.g., by
    age, gender)?} If so, please describe how these subpopulations are
  identified and provide a description of their respective
  distributions within the dataset.

\paragraph{Is it possible to identify individuals (i.e., one or
    more natural persons), either directly or indirectly (i.e., in
    combination with other data) from the dataset?} If so, please
    describe how.

\paragraph{Does the dataset contain data that might be considered
    sensitive in any way (e.g., data that reveals rac\edit{e} or ethnic
    origins, sexual orientations, religious beliefs, political
    opinions or union memberships, or locations; financial or health
    data; biometric or genetic data; forms of government
    identification, such as social security numbers, criminal
    history)?} If so, please provide a description.

\paragraph{Any other comments?}



\subsection{Collection Process}

As with the \edit{questions in the} previous section, dataset creators should
read through these questions prior to any data collection to flag
potential issues and then provide answers once the collection is complete.
\edit{In addition to the goals outlined in the previous section, the
questions in this section are designed to elicit information that may
help researchers and practitioners create alternative datasets with
similar characteristics. Again, questions that apply only to datasets
that relate to people are grouped together at the end of the
section.}\\



\paragraph{How was the data associated with each instance
    acquired?} Was the data directly observable (e.g., raw text, movie
  ratings), reported by subjects (e.g., survey responses), or
  indirectly inferred/derived from other data (e.g., part-of-speech
  tags, model-based guesses for age or language)? If \edit{the} data was reported
  by subjects or indirectly inferred/derived from other data, was the
  data validated/verified? If so, please describe how.

It was acquired by manual annotation.

\paragraph{What mechanisms or procedures were used to collect the
    data (e.g., hardware apparatus\edit{es} or sensor\edit{s}, manual human
    curation, software program\edit{s}, software API\edit{s})?} How were these
    mechanisms or procedures validated?

Manual human curation.


\paragraph{If the dataset is a sample from a larger set, what was
    the sampling strategy (e.g., deterministic, probabilistic with
    specific sampling probabilities)?}

    This dataset is not a sample from a larger set.

\paragraph{Who was involved in the data collection process (e.g.,
    students, crowd workers, contractors) and how they were compensated
    (e.g., how much were crowdworkers paid)?}

Graduate students are involved in the data collection process, and they are graduate students.

\paragraph{Over what timeframe was the data collected?} Does this
  timeframe matches the creation timeframe of the data associated with
  the instances (e.g., the recent crawl of old news articles)?  If not,
  please describe the timeframe in which the data associated with the
  instances were created.

  The timeframe in which the data associated with the instances was created is Nov. 2023.

\paragraph{Were any ethical review processes conducted (e.g., by an
    institutional review board)?} If so, please provide a description
  of these review processes, including the outcomes, as well as a link
  or other access point to any supporting documentation.

No.

\edit{If the dataset does not relate to people, you may skip the remaining questions in this section.}

The dataset does not relate to people, so we skip the remaining questions.


\paragraph{Did you collect the data from the individuals in
    question directly, or obtain it via third parties or other sources
    (e.g., websites)?}

\paragraph{Were the individuals in question notified about the data
    collection?} If so, please describe (or show with screenshots or
  other information) how notice was provided, and provide a link or
  other access point to, or otherwise reproduce, the exact language of
  the notification itself.

\paragraph{Did the individuals in question consent to the
    collection and use of their data?} If so, please describe (or show
  with screenshots or other information) how consent was requested, and
  provided, and provide a link or other access point to, or otherwise
  reproduce, the exact language to which the individuals consented.

\paragraph{If consent was obtained, were the consenting individuals
    provided with a mechanism to revoke their consent in the future or
    for certain uses?} If so, please provide a description, as well as
  a link or other access point to the mechanism (if appropriate).

\paragraph{Has an analysis of the potential impact of the dataset
    and its use on data subjects (e.g., a data protection impact
    analysis) been conducted?} If so, please provide a description of
  this analysis, including the outcomes, as well as a link or other
  access point to any supporting documentation.

\paragraph{Any other comments?}



\subsection{Preprocessing/cleaning/labeling}



Dataset creators should read through these questions prior to any
preprocessing, cleaning, or labeling and then provide answers once
these tasks are complete. The questions in this section are intended
to provide dataset consumers with the information they need to
determine whether the ``raw'' data has been processed in ways that are
compatible with their chosen tasks. For example, text that has been
converted into a ``bag-of-words'' is not suitable for tasks involving
word order.\\



\paragraph{Was any preprocessing/cleaning/labeling of the data done
    (e.g., discretization or bucketing, tokenization, part-of-speech
    tagging, SIFT feature extraction, removal of instances, processing
    of missing values)?} If so, please provide a description. If not,
  you may skip the remain\edit{ing} questions in this section.

  The dataset underwent stringent quality checks, particularly for code executability and argument accuracy, with any non-compliant data being revised or discarded. This ensures that the instructions precisely align with user requirements, thereby upholding the integrity and applicability of the ML-Bench benchmark.

\paragraph{Was the ``raw'' data saved in addition to the preprocessed/cleaned/labeled data (e.g., to support unanticipated future uses)?} If so, please provide a link or other access point to the ``raw'' data.

No.

\paragraph{Is the software \edit{that was} used to preprocess/clean/label the \edit{data} available?} If so, please provide a link or other access point.

No.

\paragraph{Any other comments?}

No.

\subsection{Uses}

\edit{The} questions \edit{in this section} are intended to encourage dataset
creators to reflect on the tasks for which the dataset should and
should not be used. By explicitly highlighting these tasks, dataset
creators can help dataset consumers make informed decisions,
thereby avoiding potential risks or harms.\\



\paragraph{Has the dataset been used for any tasks already?} If so, please provide a description.

The dataset has been used to evaluate repository-level code generation.

\paragraph{Is there a repository that links to any or all papers or systems that use the dataset?} If so, please provide a link or other access point.

No.

\paragraph{What (other) tasks could the dataset be used for?}

No.

\paragraph{Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?} For example, is there anything that a \edit{dataset consumer} might need to know to avoid uses that could result in unfair treatment of individuals or groups (e.g., stereotyping, quality of service issues) or other \edit{risks or} harms (e.g., \edit{legal risks,} financial harms\edit{)?} If so, please provide a description. Is there anything a \edit{dataset consumer} could do to mitigate these \edit{risks or} harms?

No.

\paragraph{Are there tasks for which the dataset should not be used?} If so, please provide a description.

No.

\paragraph{Any other comments?}

No.

\subsection{Distribution}

Dataset creators should provide answers to these questions prior to
distributing the dataset either internally within the entity on behalf
of which the dataset was created or externally to third parties.\\



\paragraph{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?} If so, please provide a description.

Yes. The dataset is distributed to the public.

\paragraph{How will the dataset will be distributed (e.g., tarball on website, API, GitHub)?} Does the dataset have a digital object identifier (DOI)?

GitHub. The dataset does not have a digital object identifier.

\paragraph{When will the dataset be distributed?}

The dataset is already distributed in GitHub.

\paragraph{Will the dataset be distributed under a copyright or other intellectual property (IP) license and/or under applicable terms of use (ToU)?} If so, please describe this license and/or ToU and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms or ToU, as well as any fees associated with these restrictions.

MIT license.

\paragraph{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?} If so, please describe these restrictions and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms, as well as any fees associated with these restrictions.

No.

\paragraph{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?} If so, please describe these restrictions, and provide a link or other access point to or otherwise reproduce any supporting documentation.

No.

\paragraph{Any other comments?}

No.

\subsection{Maintenance}

As with the \edit{questions in the} previous section, dataset creators
should provide answers to these questions prior to distributing the
dataset. The questions \edit{in this section} are intended to
encourage dataset creators to plan for dataset maintenance and
communicate this plan \edit{to} dataset consumers.\\



\paragraph{Who \edit{will be} supporting/hosting/maintaining the dataset?}

GitHub will be hosting the dataset..

\paragraph{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}

GitHub website.

\paragraph{Is there an erratum?} If so, please provide a link or other access point.

No.

\paragraph{Will the dataset be updated (e.g., to correct labeling
    errors, add new instances, delete instances)?} If so, please
  describe how often, by whom, and how updates will be communicated to
  \edit{dataset consumers} (e.g., mailing list, GitHub)?

No.

\paragraph{If the dataset relates to people, are there applicable
    limits on the retention of the data associated with the instances
    (e.g., were \edit{the} individuals in question told that their data would
    \edit{be} retained for a fixed period of time and then deleted)?} If so,
    please describe these limits and explain how they will be
    enforced.

The dataset does not relate to people.

\paragraph{Will older versions of the dataset continue to be
    supported/hosted/maintained?} If so, please describe how. If not,
  please describe how its obsolescence will be communicated to \edit{dataset
  consumers}.

Yes.

\paragraph{If others want to extend/augment/build on/contribute to
    the dataset, is there a mechanism for them to do so?} If so,
  please provide a description. Will these contributions be
  validated/verified? If so, please describe how. If not, why not? Is
  there a process for communicating/distributing these contributions
  to \edit{dataset consumers}? If so, please provide a description.

Yes. They can contribute by connecting to the authors. Their contributions will be verified by the authors.

\paragraph{Any other comments?}

No.

==> latex/10-checklist.tex <==
\clearpage
\newpage

\section*{NeurIPS Paper Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discussed the limitations in \autoref{sec:limitation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the experiment settings are discussed in \autoref{sec:setup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have released the code. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the details of experiment settings can be found in \autoref{sec:setup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the experiments are deterministic, and we don't have the error bars.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We mentioned the compute machine we used in \autoref{sec:setup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In \autoref{appendix:details_of_selected_github_repositries}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: It is discussed in the released code base.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> template/Agent_Step1.tex <==

\begin{table*}[h]
\centering
\begin{tabular}{p{0.98\linewidth}}
\toprule

\hline
\rowcolor{gray!20}
\textbf{Instruction}\\
\hline
Please help me extract the keywords in this sentence about the model used and the task I want to do.\\
\\
Sentence :\{\}\\
\\

\bottomrule

\end{tabular}
\caption{
The function of this prompt agent is to extract keywords about the model used and the task I want to do from the given sentence.
}
\label{table:extracting_keywords}
\end{table*}

==> template/Agent_Step2.tex <==

\begin{table*}[h]
\centering
\begin{tabular}{p{0.98\linewidth}}
\toprule

\hline
\rowcolor{gray!20}
\textbf{Instruction}\\
\hline
Sort the names and descriptions of the GitHub repositories below based on their relevance to the keywords \{keyword\}. \\
URLS:\{\}
Make sure your answer is in standard JSON format; start!
\\

\hline
\rowcolor{gray!20}
\textbf{Example}\\
\hline
Below is an example:\\
Sort the names and descriptions of the GitHub repositories below based on their relevance to the keywords \{CNN, Time-Series\}. \\
URLS:\{\\
'https://github.com/mrharicot/monodepth',\\
'https://github.com/saeedkhaki92/CNN-RNN-Yield-Prediction',\\
'https://github.com/PatientEz/CNN-BiLSTM-Attention-Time-Series-Prediction\_Keras',\\
'https://github.com/hardyqr/CNN-for-Stock-Market-Prediction-PyTorch',\\
'https://github.com/muskie82/CNN-DSO',\\
'https://github.com/gognjanovski/StockPredictionCNN',\\
'https://github.com/kristpapadopoulos/seriesnet',\\
'https://github.com/Shen-Lab/DeepAffinity',\\
'https://github.com/matheusbfernandes/stock-market-prediction',\\
'https://github.com/perseus784/Vehicle\_Collision\_Prediction\_Using\_CNN-LSTMs'\\
\}\\
Make sure your answer is in standard json format, start!\\
\\

\bottomrule

\end{tabular}
\caption{
Rank GitHub repositories related to keywords.
Sort the GitHub repository related to keywords, and the array is arranged.
}
\label{table:rank_repo_url}
\end{table*}

==> template/Agent_Step3.tex <==

\begin{table*}
\centering
\begin{tabular}{p{0.98\linewidth}}
\toprule

\hline
\rowcolor{gray!20}
\textbf{Instruction}\\
\hline
I will provide you with the name of a GitHub repository and the main README file. Please determine if you can accomplish the following task. If you can, output 'Yes' and sort the provided README files below based on their helpfulness in completing the task, from most helpful to least helpful. If you believe you cannot complete the task, please output 'No.'\\
\\
repo\_name: \{repo\_name\}
main\_README\_file: \{README\}
task: \{Instruction\}
\\

\bottomrule

\end{tabular}
\caption{
Use the information given to determine whether the task can be completed.
The given information serves as an indicator of whether the task can be completed. If it can be completed, return 'Yes'; if it cannot be completed, return 'No'. e.g., No. e.g., Yes.
Sorted list of README files based on their helpfulness in completing the task. Remember that the result must be a list! e.g.: repo\_name/README.md, repo\_name/examples/README.md, repo\_name/scripts/atlas/README.md.
}
\label{table:evaluation_task}
\end{table*}

==> template/Agent_Step4.tex <==

\begin{table*}[h]
\centering
\begin{tabular}{p{0.98\linewidth}}
\toprule

\hline
\rowcolor{gray!20}
\textbf{Instruction}\\
\hline
  I will provide you with a GitHub README file and directory index; please determine if this information is enough to write the code or script for the task I gave you. Write the code or script directly if you can, give us the path to the py file you want from the repository index file if you need more information. Please make sure that the file path you return is in the repository index file!!! And return NO if you don't think all of this information will do the job.\\
  repository\_index\_file:\{\}\\
  README file:\{\}\\
  task:\{\}\\
\\

\bottomrule

\end{tabular}[h]
\caption{
Code that uses given information to determine whether or not it can accomplish a given task.
}
\label{table:evaluation_readme}
\end{table*}

==> template/FT_LM.tex <==

\begin{table*}[h]
\centering
\caption{Formatting structure for README and instruction inputs in fine-tuning.}
\begin{tabular}{p{0.98\linewidth}}
\toprule

\hline
\rowcolor{gray!20}
\textbf{README}\\
\hline
[readme]:\{README\}\\
\\
\hline
\rowcolor{gray!20}
\textbf{Instruction}\\
\hline
[instruction]:\{Instruction\}\\
\\

\bottomrule

\end{tabular}
\label{table:template_ft_lm}
\end{table*}

==> template/LLM.tex <==

\begin{table*}[h]
\centering
\caption{Template for LLM's prompt, README, and instruction input format}
\begin{tabular}{p{0.98\linewidth}}
\toprule
\hline
\rowcolor{gray!20}
\textbf{System Prompt}\\
\hline
You are given [readme], you need to carefully see [readme] and choose to write code or script to implement my [instruction]. \\
Please output your response in a Python markdown code block.\\
\\
\hline
\rowcolor{gray!20}
\textbf{README}\\
\hline
[readme]:\{README\}\\
\\
\hline
\rowcolor{gray!20}
\textbf{Instruction}\\
\hline
[instruction]:\{Instruction\}\\
\\

\bottomrule

\end{tabular}
\label{table:template_llm}
\end{table*}
